Robust Social Welfare Maximization via Information Design in Linear-Quadratic-Gaussian Games

Information design in an incomplete information game includes a designer with the goal of influencing players' actions through signals generated from a designed probability distribution so that its objective function is optimized. We consider a setting in which the designer has partial knowledge on agents' utilities. We address the uncertainty about players' preferences by formulating a robust information design problem against worst case payoffs. If the players have quadratic payoffs that depend on the players' actions and an unknown payoff-relevant state, and signals on the state that follow a Gaussian distribution conditional on the state realization, then the information design problem under quadratic design objectives is a semidefinite program (SDP). Specifically, we consider ellipsoid perturbations over payoff coefficients in linear-quadratic-Gaussian (LQG) games. We show that this leads to a tractable robust SDP formulation. Numerical studies are carried out to identify the relation between the perturbation levels and the optimal information structures.

==> introduction.tex <==
Information design refers to the determination of the information fidelity of the signals given to the players in an incomplete information game, so that the induced actions of players maximize a system level objective \cite{Bergemann2019}.  In an incomplete information game, players compete to maximize their individual payoffs that depend on the action of the player, other players' actions and an unknown state. Incomplete information games are used to model power allocation of users in wireless networks with unknown channel gains \cite{bacci2015game}, traffic flow in communication or transportation networks \cite{wu2021value}, and currency attacks of investors \cite{morris2002social}. In this research, we envision the existence of an information designer that can provide the ``best'' information about the payoff-relevant states to the players according to its design objective. 

Information design originated from Bayesian persuasion framework which involves a sender, i.e. information designer and a single receiver, i.e. agent. The goal is to maximize sender's objective by persuading a  rational agent regarding a payoff state affecting receiver's utility via revealing credible information \cite{Kamenica2011}. In multi-player systems, information designer aims to optimize a system level objective, such as social welfare, by selecting an information structure, and the corresponding induced rational behavior of multiple agents to overcome undesirable or inefficient outcomes \cite{Bergemann2013,Bergemann2019}. In general, the designer's problem is computationally intractable as it involves identifying the ``best'' distribution over the space of distributions that induces desirable rational behavior \cite{Dughmi2017}. Thus, the current approaches make structural assumptions about the state/action space, the system designer's objective, and the game payoffs in order to attain analytical results \cite{candogan2020information}. 

\begin{figure}[h]
\centering
\begin{tikzpicture}[scale=1]
\Vertex[size=1.3,x=0.5,y=0.5]{A} 
\Vertex[size=1.3, x=2.5,y=-1.5, color=magenta]{B}
\Vertex[size=1.3, x=-2.5,y=-1.5, color=magenta]{C}
\Vertex[size=1.3,, x=3,y=1.5]{D}
\Vertex[size=1.3, x=-3,y=1.5, color=green]{E}
\Vertex[size=1.3,x=-0.7,y=-1.5, color=green]{G}
\Text[fontsize=\footnotesize,width=1.2cm,x=0.5,y=0.5]{Agent 1}
\Text[fontsize=\footnotesize,width=1.2cm,x=2.5,y=-1.5]{Agent 2} 
\Text[fontsize=\footnotesize,width=1.2cm,x=-2.5,y=-1.5]{Agent 3}
\Text[fontsize=\footnotesize,width=1.2cm,x=3,y=1.5]{Agent 4}
\Text[fontsize=\footnotesize,width=1.2cm, x=-3,y=1.5]{Agent 5}
\Text[fontsize=\footnotesize,width=1.2cm, x=-0.7 ,y=-1.5]{Agent 6}
\Vertex[size=1.8, y=3, color=yellow ]{F}
\Text[fontsize=\footnotesize,width=1.5cm,x=0, y=3]{Information Designer}
\Edge(A)(B)
\Edge(A)(C)
\Edge(A)(D)
\Edge(A)(E)
\Edge(E)(B)
\Edge(C)(G)
\Edge(G)(D)
\Edge[color=red](A)(F)
\Edge[color=red](F)(B)
\Edge[color=red](F)(C)
\Edge[color=red](F)(D)
\Edge[color=red](F)(E)
\Edge[color=red](F)(G)
\end{tikzpicture}
\caption{Information designer sends optimally designed signals on the risks of infection from an emerging infectious disease to the population with individuals who are susceptible (blue), infected (green) or recovered (magenta), so that they follow the recommended health measures, e.g. social distancing or masking that reduce the risk of an outbreak. An individual's infection or disease transmission risk is determined by its contacts (shown by black edges). For instance agent 1 (susceptible) has one infected neighbor (agent 5) that it can contract the disease from.}
\label{inf_design_diagram_epidemic}
\vspace{-12pt}
\end{figure} 

To further illustrate the information design problem, we consider an example from pandemic control (see Fig. \ref{inf_design_diagram_epidemic}). Consider a public health institute, e.g., Centers for Disease Control and Prevention (CDC) or a local health department, that determines the fidelity of information revealed about the unknown risks of an emerging infectious disease, in order to eliminate or reduce the risks of an outbreak. The agents in the population can be in  susceptible, infected, and recovered states. A susceptible agent determines its level of adherence to recommended preventative health measures based on its assessment of risks of an infection, and costs of the measures. For instance, both susceptible agents (agent 1 and 4) have a single infected contact (agent 5 and 6) that they can contract the disease from (shown by black lines in Fig. \ref{inf_design_diagram_epidemic}). An infectious agent pits the risks associated with transmitting the disease to other agents against the costs of taking the isolation measures. For instance, both infected agents (agent 5 and 6) have one susceptible and one recovered contact. The higher is the number of susceptible contacts, the stronger is the risk for disease transmission. A local health department (designer) has more information about the potential risks associated with an emerging infectious disease. Its goal is to induce actions that will reduce the disease transmission in the population by sending signals on infection risk or campaigning for certain actions, e.g., social distancing, or masking indoors. In this setting, the health department has to reveal credible information based on the actual (realized) severity of the infectious disease. 

\subsection{Contributions}
In this paper, we propose a robust optimization approach to the information design problem considering the fact that the designer cannot exactly know the game players are in. Indeed, while the designer may be knowledgeable about the payoff relevant random state, it may have uncertainty about the payoff coefficients of the players. For instance, in the pandemic control example above while the public health department may have near-certain information about the potential risks of a disease or intervention, it may not know how the society weights the risks and benefits in their decision-making. Here, we assume the designer has partial knowledge about players' utilities, and wants to perform information design over the payoff relevant states. 

When the payoffs of the players are unknown, the designer cannot be sure of the rational behavior under a chosen information structure. We formulate this problem as a robust optimization problem where the designer chooses the ``best'' optimal information structure for the worst possible realization of the payoffs. That is, we do not make any assumptions on the distribution of the players' payoff coefficients.  

Specifically, we assume the players have linear-quadratic payoffs with coefficients unknown by the designer. We further assume that the payoff relevant states and signals generated by the designer come from a Gaussian distribution. In this setting, we show that the robust information design problem can be formulated as a tractable SDP given ellipsoid, interval or general cone perturbations on the payoff coefficients--see Theorem \ref{theorem_model} and supplementary materials. Using the tractable SDP formulation under ellipsoid perturbations, we establish the optimality of canonical information disclosure settings, namely no and full information disclosure, given the set of general (Theorem \ref{theorem_general}) and public (Theorem \ref{theorem_pub_no} and \ref{theorem_full}) information structures. 
% In information design literature \cite{Bergemann2013,Bergemann2019,Ui2020}, it is assumed that information designer has full information over players' utilities, i.e. it knows the payoff functions exactly. This assumption is not realistic from privacy and data communication perspectives. Constant payoff coefficients are different from the payoff state which is governed by a probability distribution. Also, information design is on selecting an information structure for the payoff state. 
% In contrast, we consider a realistic setting in which the designer has partial knowledge on agents' utilities and still needs to perform information design over payoff state. We address the uncertainty about player's preferences by formulating a robust information design problem. 

% Specifically, we consider ellipsoid perturbations over payoff matrices in LQG games. We aim to show that this leads to a robust SDP formulation. Using the robust SDP formulation, we obtain analytical conditions for the optimality of no information and full information disclosure. We note that the robust convex program can also be extended to general convex cone and interval uncertainties about the payoff matrices. Numerical studies is carried out to identify the relation between the perturbation levels and the optimal information structures.


% \cite{dworczak2022preparing} considers the situation where the nature also provides information on payoff state to the receiver, i.e., agent to minimize the sender’s payoff, i.e., information designer's objective. They still assume agents' utilities are known by the designer.  Similar to \cite{dworczak2022preparing}, \cite{hu2021robust} consider the same setting that receiver is informed by Nature and identify optimal information structures. Our work differentiates from them because we do not consider the Nature as an entity and we assume partially known agents' utilities by the designer.
% \cite{zu2021learning} considers the situation where the sender does not know the prior distribution on payoff state and the sender learns it in a repeated persuasion setting. The sender aims to minimize regret with respect to the setting where the sender knows the prior distribution on payoff state. Our paper considers a static information design setting and we assume prior distribution on payoff state is known by the designer. 
% \cite{BABICHENKO2022226} considers an adversarial approach to robust Bayesian persuasion under unknown utility problem with the goal of minimizing regret over a single persuasion instance. Their robustness considerations is with respect to agents' utilities as ours. However, they focus on an regret minimizing framework whereas our focus is robust information design under perturbed utilities. The designer knows the perturbed utilities in our case. However, it does not know the amount of perturbation. 
% Finally, \cite{deClippel2022} studies robustness against the situation that the receiver calculates the posterior distribution of payoff state up to some error after receiving the signal from the sender. We assume the receiver is capable to calculate posterior without error.


\subsection{Techniques}
We build on the SDP formulation for information design in LQG games with known payoffs \cite{Ui2020}. This SDP formulation entails a  set of linear equalities that represent the Bayesian correlated equilibrium (BCE) conditions. In the robust optimization approach these conditions are not exactly satisfied by some of the payoff realizations. After establishing the deviation in these constraints for a finite scenario setting, we derive the robust counterparts of these BCE constraints under ellipsoid (Section \ref{sec_trac}), interval (Supplementary Material \ref{sec_int}) and general cone (Supplementary Material \ref{sec_cone}) perturbations to agents' utilities.
% We write robust counterparts of the constraints of the SDP affected by ellipsoid (section \ref{sec_trac}), interval (appendix \ref{sec_int}) and general cone (appendix \ref{sec_cone}) perturbations to agents' utilities. Thus, we build robust convex optimization models of information design under perturbed utilities in LQG games. 
We also showcase how to proceed if perturbations affect the objective as in the case social welfare objective, by rewriting the designer's objective as a constraint, and building a robust constraint for it. 

After formulating the tractable SDPs, we establish sufficient conditions for the optimality of no and full information disclosure under ellipsoid uncertainty in Section \ref{sec_res}. These results provide conditions on the perturbation set radius and the eigenvalues of the perturbed payoff coefficients for the optimality of the extreme information structures. In numerical examples, we show that as the designer's uncertainty about the players' utilities grows, the optimal information structure approaches no information disclosure. 
% In section \ref{sec_nume}, we implement our robust convex optimization model with social welfare objective under ellipsoid perturbations and feed it into a convex optimization solver to analyze optimal information structures under a spectrum of perturbation levels.
% Defining information design problem over action distribution renders possible to define the problem as a semi-definite program (SDP).  Non-robust version of the SDP, that is no minimization over strategies, is tractable \cite{sezer2021social}. }


\subsection{Literature Review}
It is worth noting that there are existing works in the framework of Bayesian persuasion and information design that consider robustness in a different sense than our framework. Both \cite{dworczak2022preparing} and \cite{hu2021robust} consider the Bayesian persuasion setting with a sender and a receiver agents, where the nature may send additional information to the receiver, and aim to find the sender's optimal information structures. These works assume the receiver's payoff is known by the sender, but consider robustness against the side information provided by the nature to the receiver. 

In another Bayesian persuasion setting, \cite{zu2021learning} considers the situation where the sender does not know the prior distribution on payoff state and the sender learns it over repeated interactions. The goal of the sender is to minimize regret with respect to the setting where the sender knows the prior distribution on payoff state. Their main result proves that for any persuasion setting satisfying certain regularity conditions, their proposed algorithm achieves $O (\sqrt{T \log T})$ regret with high probability under the horizon length $T$. In contrast, here we consider a one-shot (static) problem, and we assume the prior distribution on the payoff state is known by the designer.


In \cite{BABICHENKO2022226}, an adversarial approach is taken for the setting where the sender does not know the utility of the receiver. That is, the robustness is against the unknown receiver utilities similar to ours. They show that the sender can achieve a low regret under the assumption that it knows the receiver's ordinal preferences over the states of nature upon adoption. However, they formulate the problem as regret minimizing, whereas we formulate the problem using robust optimization. The difference is that we assume the designer knows the perturbed payoff functions, but it does not know the amount of perturbation. Lastly, robustness against the receiver's error prone (non-Bayesian probabilistic inference over payoff state) calculations is considered in \cite{deClippel2022}. In our case, we assume the receiving agents are capable of updating their expected payoffs without error. 

Besides the mentioned distinctions between our framework and  \cite{dworczak2022preparing,hu2021robust,zu2021learning,BABICHENKO2022226,deClippel2022}, we focus on the multi-player setting, i.e., information design, and assume an incomplete information game among the players.

% Information design literature takes its roots from Bayesian persuasion with \cite{Kamenica2011}. Bayesian persuasion framework assumes a sender i.e information designer and single Bayesian rational receiver i.e agent. Information design supersedes Bayesian persuasion with an information designer and multiple agents who play an incomplete information game among themselves \cite{Bergemann2013,Bergemann2019}. The solution concept of the game is Bayesian correlated equilibrium which an information structure should satisfy so that agents will follow the recommended action or signal from the designer. 
% Studies in robust information design and Bayesian persuasion employs various robustness definitions. \cite{dworczak2022preparing} develops worst case robust solutions for the sender against Nature which provides information to receiver to minimize sender's payoff. In the privately informed receivers setting, \cite{hu2021robust}  characterize optimal information structures from the class of linear-contingent-payoff information structures and show that it is suffice to consider only this class of information structures for optimal persuasion.
% \cite{zu2021learning} assumes the sender does not know prior distribution of payoff state initially and it is learning it over time in repeated setting. The goal of the sender is to minimize the regret compared to situation that the sender knows the prior distribution. Their main result proves that for any persuasion setting satisfying certain regularity conditions, their algorithm achieves $O (\sqrt{T \log T})$ regret with high probability under the horizon length $T.$ 

% \cite{BABICHENKO2022226} consider regret minimizing persuasion under unknown utilities. They show that the sender can achieve a low regret under the assumption that it knows the receiver's ordinal preferences over the states of nature upon adoption.  In contrast to these papers, our paper develops robust convex optimization models for information design under perturbed utilities, i.e our robustness is against perturbed utilities.

% \cite{deClippel2022} consider non-Bayesian probabilistic inference over payoff state. Under robust setting, they assume an uncertainty ball over possible posteriors of payoff state. Their main result on robust Bayesian persuasion states that uncertainty ball over posteriors reduces to a distortion function under worst posterior for the sender.
 
Information design in operations gained importance recently, see \cite{candogan2020information} for a detailed review. 
On further development of information design methodology, \cite{koessler2022} presents equilibrium existence results when there are competing information designers, and \cite{gradwohl2022} develops approximation algorithms for persuasion under limited communication. 
%
In revenue maximization, \cite{emek2014} studies optimal signalling mechanism in second price auctions. Value of personalized information provisioning compared to public information is studied by \cite{drakopoulos2021persuading}. \cite{kucukgul2022time} presents results on optimal information policy in time-locked sales.
In queuing systems, \cite{lingenbrink2019} considers a designer who gives information on state of the queue to customers to maximize expected revenue. \cite{Heydaribeni2021} considers information design in queues where customers make a payment to learn the signal regarding the state of the queue. In public health management, informing the public about approaching health emergencies such as epidemics \cite{alizamir2020healthcare} and workplace occupancy control, i.e., in person vs remote via informing about infection risk parameter \cite{shah2022optimal} is studied. In platform management, nudging suppliers to use platform is studied by \cite{bimpikis2022stra}. \cite{gur2022information} studies an e-commerce platform as a designer who studies joint promotion and information policy in e-commerce platforms. In \cite{candogan2020signaling}, the authors  identify networks that are amenable to persuasion in a setting where designer provides post recommendations to users.

 %It focuses on public information structures and identifies which networks are more amenable to persuasion. \blue{In a reverse perspective, \cite{sezer2022} assesses the benefit of optimal information design to the players in a network game by characterizing the utility gain of the players from information disclosure based on their position (centrality) in the network.}



